Linear Projections of Teacher Embeddings for Few-Class Distillation

Knowledge Distillation (KD) has emerged as a promising approach for transferring knowledge from a larger, more complex teacher model to a smaller student model. Traditionally, KD involves training the student to mimic the teacher's output probabilities, while more advanced techniques have explored guiding the student to adopt the teacher's internal representations. Despite its widespread success, the performance of KD in binary classification and few-class problems has been less satisfactory. This is because the information about the teacher model's generalization patterns scales directly with the number of classes. Moreover, several sophisticated distillation methods may not be universally applicable or effective for data types beyond Computer Vision. Consequently, effective distillation techniques remain elusive for a range of key real-world applications, such as sentiment analysis, search query understanding, and advertisement-query relevance assessment. Taking these observations into account, we introduce a novel method for distilling knowledge from the teacher's model representations, which we term Learning Embedding Linear Projections (LELP). Inspired by recent findings about the structure of final-layer representations, LELP works by identifying informative linear subspaces in the teacher's embedding space, and splitting them into pseudo-subclasses. The student model is then trained to replicate these pseudo-classes. Our experimental evaluation on large-scale NLP benchmarks like Amazon Reviews and Sentiment140 demonstrate the LELP is consistently competitive with, and typically superior to, existing state-of-the-art distillation algorithms for binary and few-class problems, where most KD methods suffer.

==> algorithms/lelp_main.tex <==
\begin{algorithm*}[t]
\small
   \caption{Learning Embedding Linear Projections (LELP)}
   \label{alg:LELP_train_main}
\begin{algorithmic}
   \STATE {\bfseries Input:} Teacher model feature extractor $h^\text{Teacher}(x)$\\
   \quad\quad\quad $C$ class mean vectors $M = \{\mu_c\}$ and $C \times S$ subclass projection vectors $\tilde{V} = \{\tilde{v}_{c,s }\}$ \\ 
    \quad\quad\quad Teacher final layer classification weights $W = [w_1 \dots w_C] \in R^{D\times C}$ and biases $[b_1 \dots b_C]$\\
    \quad\quad\quad Subclass Temperature and Student-Teacher temperatures $\beta, \tau$ \\
    \quad\quad\quad $C\times S$ class student model $f_{\theta_S}^\text{Student}(x)$ and weights $\theta_S$\\
    \quad\quad\quad Dataset $p(x)$, Learning rate $\eta$ \\
   \STATE {\bfseries Output:} Trained Student Model $\theta$
   \WHILE {Not converged}
        \STATE Sample $x \sim p(x)$
        \STATE Compute teacher embedding $h^\text{Teacher} \leftarrow h^\text{Teacher}(x)$
        \STATE Compute teacher subclass probabilities $p^\text{Teacher}_{s,c} \leftarrow \texttt{subsplit}(h, \tilde{V}, M, W, \beta, \tau)$ (See \cref{alg:pseudo_class_split} in \cref{app:alg_details})
        \STATE Compute $C\times S$ student logits: $z^\text{Student}_{c,s} \leftarrow f^\text{Student}_{\theta_S}(x)$
        \STATE Compute $C\times S$ tempered student probabilities: $p_{c, s}^\text{Student} \leftarrow \frac{e^{z^\text{Student}_{c, s}/\tau}}{\sum_{i = 1}^C\sum_{j = 1}^S e^{z^\text{Student}_{i, j}/\tau}}$
        \STATE Compute LELP loss $\mathcal{L}_{LELP} = \tau^2 \sum_{c = 1}^C\sum_{s = 1}^S p^\text{Teacher}_{c,s} \log\frac{p^\text{Teacher}_{c,s}}{p^\text{Student}_{c,s}}$ (Standard KL Divergence)
        \STATE Update student parameters: $\theta_S \leftarrow \theta_S - \eta \frac{\partial \mathcal{L}_{LELP}}{\partial \theta_S}$
   \ENDWHILE
   \STATE {\bfseries Return: } $\theta_S$
\end{algorithmic}
\end{algorithm*}

==> tables/binary_with_subclass_structure.tex <==
% \begin{table*}[h] 
% \renewcommand{\arraystretch}{1.15}
% \caption{Experiments on \textbf{Vision Binary Classification tasks with subclass structure}.}
% \label{tab:binary-subclass-structure}

% \begin{center}
% \tiny
% \begin{tabular}{|c| c c c c |} 
%  \hline
%  %\rowcolor{cyan}
% \cellcolor{cyan}
% Teacher Architecture & ResNet92 & ResNet92  & ResNet92  & ResNet92 \\ 

%  \hline
%  % \rowcolor{cyan}
%  \cellcolor{cyan}
% Student Architecture  & ResNet56 &  MobileNet  & ResNet56  & MobileNet \\ 
% \hline
%  \cellcolor{cyan}
% Dataset&

% CIFAR-10-bin&  
% CIFAR-10-bin& 
% CIFAR-100-bin& 
% CIFAR-100-bin \\ 
% \hline
%  \cellcolor[HTML]{FBB982}
%  Teacher & 
%  $ 96.70$ &  
%  $96.70$ & 
%  $ 78.69 $ & 
%  $ 78.69$ \\
% \hline
%  \cellcolor[HTML]{FBB982}
%  Subclass Distillation Teacher
%  & 
%  $ 96.12 $ &  
%  $95.99 $ & 
%  $ 77.52 $ & 
%  $ 75.87 $ \\
% \hline
%  \cellcolor[HTML]{FBB982}
% Oracle Clustering & 
%  $ 97.17 \pm 0.02$ &  
%  $93.23 \pm 0.28 $ & 
%  $ 86.42 \pm 0.11 $ & 
%  $ 76.59 \pm 0.60$ \\
% \hline
% \cellcolor[HTML]{FDBC42}
% Standard Training & 
%  $ 95.43 \pm 0.07$ &  
%  $ 92.04 \pm 0.26 $ & 
%  $ 74.80 \pm 0.52 $ & 
%  $ 69.13 \pm 0.32$ \\
 
%  \hline
% \cellcolor[HTML]{FDBC42}
%  Vanilla Distillation~\cite{distillation} & 
%  $ 95.75 \pm 0.21$ &  
%  $ 92.91 \pm 0.17 $ & 
%  $ 72.87 \pm 0.27 $ & 
%  $ 72.16 \pm 0.39$ \\
 
%  \hline
%  \cellcolor[HTML]{FDBC42}
%  Embedding Distillation &   
%  $96.48 \pm 0.1$  & 
%  $93.05 \pm 0.13$ & 
%  $78.77 \pm 0.35$ & 
%  $72.24 \pm 0.20$ \\
 
%  \hline
%  \cellcolor[HTML]{FDBC42}
%  FitNet~\cite{romero2014fitnets} &   
%  $ 96.53 \pm 0.05$ & 
%  $ 93.31 \pm 0.11$ & 
%  $ 79.14 \pm 0.18$ & 
%  $  71.76 \pm 0.26 $\\
%  \hline
%  \cellcolor[HTML]{FDBC42}
%  VID \cite{Ahn2019CVPR} & 
%  $96.13 \pm 0.16$ & 
%  $89.95 \pm 1.34$ & 
%  $75.69 \pm 0.55$ & 
%  $71.99 \pm 0.18$ \\  
%  \hline
%  \cellcolor[HTML]{FDBC42}
%  Subclass Distillation \cite{muller2020subclass} &  
%  $96.44 \pm 0.06$ & 
%  $93.76 \pm 0.06$ & 
%  $79.23 \pm 0.17$ & 
%  $73.90 \pm 0.18$ \\
%  \hline
%  \cellcolor[HTML]{FDBC42}
% LELP (Ours) &  
%  $\mathbf{96.71 \pm 0.04}$ & 
%  $\mathbf{93.99 \pm 0.17}$ & 
%  $\mathbf{79.91 \pm 0.15}$ & 
%  $\mathbf{75.21 \pm 0.12}$ \\
%  \hline
%   \cellcolor{lightgray}
%  Avg. gain over the best baseline &
% \cellcolor{green} $0.23$ & 
% \cellcolor{green} $0.23$ & 
% \cellcolor{green} $0.68$ & 
% \cellcolor{green} $1.31$ \\
%   \hline
% \cellcolor{lightgray}
%  Avg. gain over Vanilla KD &
% \cellcolor{green} $0.96$ & 
% \cellcolor{green} $1.08$ & 
% \cellcolor{green} $7.04$ & 
% \cellcolor{green} $3.05$ \\
%   \hline
  
% \end{tabular}
% \end{center}


% \end{table*}



% \begin{table*}[h] 
% \renewcommand{\arraystretch}{1.15}
% \caption{Experiments on \textbf{Vision Binary Classification tasks with subclass structure}.}
% \label{tab:binary-subclass-structure}

% \begin{center}
% \tiny
% \begin{tabular}{|c| c c c c |} 
%  \hline
%  %\rowcolor{cyan}
% \cellcolor{cyan}
% Teacher Architecture & ResNet92 & ResNet92  & ResNet92  & ResNet92 \\ 

%  %\hline
%  % \rowcolor{cyan}
%  \cellcolor{cyan}
% Student Architecture  & ResNet56 &  MobileNet  & ResNet56  & MobileNet \\ 
% %\hline
%  \cellcolor{cyan}
% Dataset&

% CIFAR-10-bin&  
% CIFAR-10-bin& 
% CIFAR-100-bin& 
% CIFAR-100-bin \\ 
% \hline
%  \cellcolor[HTML]{FBB982}
%  Teacher & 
%  $ 96.70$ &  
%  $96.70$ & 
%  $ 78.69 $ & 
%  $ 78.69$ \\
% %\hline
%  \cellcolor[HTML]{FBB982}
%  Subclass Distillation Teacher
%  & 
%  $ 96.12 $ &  
%  $95.99 $ & 
%  $ 77.52 $ & 
%  $ 75.87 $ \\
% %\hline
%  \cellcolor[HTML]{FBB982}
% Oracle Clustering & 
%  $ 97.17 \pm 0.02$ &  
%  $93.23 \pm 0.28 $ & 
%  $ 86.42 \pm 0.11 $ & 
%  $ 76.59 \pm 0.60$ \\
% \hline
% \cellcolor[HTML]{FDBC42}
% Standard Training & 
%  $ 95.43 \pm 0.07$ &  
%  $ 92.04 \pm 0.26 $ & 
%  $ 74.80 \pm 0.52 $ & 
%  $ 69.13 \pm 0.32$ \\
 
%  %\hline
% \cellcolor[HTML]{FDBC42}
%  Vanilla Distillation& 
%  $ 95.75 \pm 0.21$ &  
%  $ 92.91 \pm 0.17 $ & 
%  $ 72.87 \pm 0.27 $ & 
%  $ 72.16 \pm 0.39$ \\
 
% % \hline
%  \cellcolor[HTML]{FDBC42}
%  Embedding Distillation &   
%  $96.48 \pm 0.1$  & 
%  $93.05 \pm 0.13$ & 
%  $78.77 \pm 0.35$ & 
%  $72.24 \pm 0.20$ \\
 
% % \hline
%  \cellcolor[HTML]{FDBC42}
%  FitNet&   
%  $ \underline{96.53 \pm 0.05}$ & 
%  $ 93.31 \pm 0.11$ & 
%  $ 79.14 \pm 0.18$ & 
%  $  71.76 \pm 0.26 $\\
%  %\hline
%  \cellcolor[HTML]{FDBC42}
%  VID  & 
%  $96.13 \pm 0.16$ & 
%  $89.95 \pm 1.34$ & 
%  $75.69 \pm 0.55$ & 
%  $71.99 \pm 0.18$ \\  
% % \hline
%  \cellcolor[HTML]{FDBC42}
%   Relational KD  & 
%  $96.22 \pm 0.09$ & 
%  $92.98 \pm 0.21$ & 
%  $78.57 \pm 0.64$ & 
%  $72.53 \pm 0.23$ \\  
% % \hline
%  \cellcolor[HTML]{FDBC42}
%  Subclass Distillation  &  
%  $96.44 \pm 0.06$ & 
%  $\underline{93.76 \pm 0.06}$ & 
%  $\underline{79.23 \pm 0.17}$ & 
%  $\underline{73.90 \pm 0.18}$ \\
% % \hline
%  \cellcolor[HTML]{FDBC42}
% LELP (Ours) &  
%  $\mathbf{96.71 \pm 0.04}$ & 
%  $\mathbf{93.99 \pm 0.17}$ & 
%  $\mathbf{79.91 \pm 0.15}$ & 
%  $\mathbf{75.21 \pm 0.12}$ \\
%  \hline
%   \cellcolor{lightgray}
%  Avg. gain over the best baseline &
% \cellcolor{green} $0.23$ & 
% \cellcolor{green} $0.23$ & 
% \cellcolor{green} $0.68$ & 
% \cellcolor{green} $1.31$ \\
% %  \hline
% \cellcolor{lightgray}
%  Avg. gain over non-subclass baseline &
% \cellcolor{green} $0.23$ & 
% \cellcolor{green} $0.68$ & 
% \cellcolor{green} $0.77$ & 
% \cellcolor{green} $2.68$ \\
%  % \hline
% \cellcolor{lightgray}
%  Avg. gain over Vanilla KD &
% \cellcolor{green} $0.96$ & 
% \cellcolor{green} $1.08$ & 
% \cellcolor{green} $7.04$ & 
% \cellcolor{green} $3.05$ \\
%   \hline
  
% \end{tabular}
% \end{center}


% \end{table*}




\begin{table*}[t] 
\centering
\renewcommand{\arraystretch}{1.15}
\caption{Warmup: Experiments on Binary Classification tasks \textbf{with Subclass Structure}.}
\label{tab:binary-subclass-structure}
\begin{center}
\tiny
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{|c| c c c c c c |} 
 \hline
 %\rowcolor{cyan}
\cellcolor{cyan}
Teacher Architecture & ResNet92 & ResNet92  & MobileNetWD2 & ResNet92  & ResNet92 & MobileNetWD2 \\ 

 %\hline
 % \rowcolor{cyan}
 \cellcolor{cyan}
Student Architecture  & ResNet56 &  MobileNet  & MobileNet &  ResNet56  & MobileNet & MobileNet \\ 
%\hline
 \cellcolor{cyan}
Dataset&

CIFAR-10-bin&  
CIFAR-10-bin& 
CIFAR-10-bin& 
CIFAR-100-bin& 
CIFAR-100-bin& 
CIFAR-100-bin \\ 
\hline
 \cellcolor[HTML]{FBB982}
 Teacher & 
 $ 96.70$ &  
 $96.70$ & 
  $93.90 $ &
 $ 78.69 $ & 
 $ 78.69$ &
  $ 72.63$ 
 \\
%\hline
 \cellcolor[HTML]{FBB982}
 Subclass Distillation Teacher
 & 
 $ 96.12 $ &  
 $95.99 $ & 
 $93.82$ &
 $ 77.52 $ & 
 $ 75.87 $ &
 $71.53 $ \\
%\hline
 \cellcolor[HTML]{FBB982}
Oracle Clustering & 
 $ 97.17 \pm 0.02$ &  
 $93.48 \pm 0.05 $ & 
 $93.48 \pm 0.05 $ &
 $ 86.59 \pm 0.05 $ & 
 $ 86.38 \pm 0.06$ &
 $ 86.38 \pm 0.06$
 \\
\hline
\cellcolor[HTML]{FDBC42}
Standard Training & 
 $ 95.43 \pm 0.07$ &  
 $ 92.04 \pm 0.26 $ & 
 $ 92.13  \pm 0.17 $ &
 $ 74.80 \pm 0.52 $ & 
 $ 69.13 \pm 0.32$ &
 $ 68.84 \pm 0.97 $ \\
 
 %\hline
\cellcolor[HTML]{FDBC42}
 Vanilla Distillation& 
 $ 95.75 \pm 0.21$ &  
 $ 92.91 \pm 0.17 $ &
  $ 92.79 \pm 0.3 $ &
 $ 72.87 \pm 0.27 $ & 
 $ 72.16 \pm 0.39$ &
$ 71.45 \pm 0.59 $ \\
 
% \hline
 \cellcolor[HTML]{FDBC42}
 Embedding Distillation &   
 $96.48 \pm 0.1$  & 
 $93.05 \pm 0.13$ & 
 $ 92.57 \pm 0.06 $&
 $78.77 \pm 0.35$ & 
 $72.24 \pm 0.20$ &
$ \underline{71.99 \pm 0.30 }$
 \\
 
% \hline
 \cellcolor[HTML]{FDBC42}
 FitNet&   
 $ \underline{96.53 \pm 0.05}$ & 
 $ 93.31 \pm 0.11$ & 
 $ 92.72 \pm 0.1 $ &
 $ 79.14 \pm 0.18$ & 
 $  71.76 \pm 0.26 $ &
 $ 68.79 \pm 2.82$
 \\
 %\hline
 \cellcolor[HTML]{FDBC42}
 VID  & 
 $96.13 \pm 0.16$ & 
 $89.95 \pm 1.34$ & 
 $84.09 \pm 3.38$ &
 $75.69 \pm 0.55$ & 
 $71.99 \pm 0.18$ & 
 $61.15 \pm 0.40 $\\  
% \hline
 \cellcolor[HTML]{FDBC42}
  Relational KD  & 
 $96.22 \pm 0.09$ & 
 $92.98 \pm 0.21$ & 
 $\underline{92.81 \pm 0.14}$ &
 $78.57 \pm 0.64$ & 
 $72.53 \pm 0.23$ & 
 $71.66 \pm 0.1$\\  
% \hline
 \cellcolor[HTML]{FDBC42}
  DKD  & 
  $95.75 \pm 0.21$ & 
  $92.91 \pm 0.17$ & 
  $92.79 \pm 0.3$ &
  $72.87 \pm 0.27$ & 
  $72.16 \pm 0.39$ & 
  $71.45 \pm 0.59$  \\  
 \cellcolor[HTML]{FDBC42}
  CRD  & 
 $ 95.83 \pm 0.25$ & 
 $92.47 \pm 0.13$ & 
 $ 92.34 \pm 0.18$ &
  $73.01 \pm 0.21 $ & 
 $72.15 \pm 0.63$ & 
 $69.53 \pm  1.37$ \\  


 \cellcolor[HTML]{FDBC42}
 Subclass Distillation  &  
 $96.44 \pm 0.06$ & 
 $\underline{93.76 \pm 0.06}$ & 
  $ 92.77 \pm 0.15$  &
 $\underline{79.23 \pm 0.17}$ & 

 $\underline{73.90 \pm 0.18}$ &
 $70.60 \pm 0.27$
 \\
% \hline
 \cellcolor[HTML]{FDBC42}
LELP (Ours) &  
 $\mathbf{96.71 \pm 0.04}$ & 
 $\mathbf{93.99 \pm 0.17}$ & 
 $ \mathbf{93.03 \pm 0.1 }$ &
 $\mathbf{79.91 \pm 0.15}$ & 
 $\mathbf{75.21 \pm 0.12}$ & 
 $ \mathbf{72.38 \pm 0.24}$\\
 \hline
  \cellcolor{lightgray}
 Avg. gain over the best baseline &
\cellcolor{green} $0.23$ & 
\cellcolor{green} $0.23$ &
\cellcolor{green} $0.22$ &
\cellcolor{green} $0.68$ & 
\cellcolor{green} $1.31$ &
\cellcolor{green} $0.39$\\
%  \hline
\cellcolor{lightgray}
 Avg. gain over non-subclass baseline &
\cellcolor{green} $0.23$ & 
\cellcolor{green} $0.68$ & 
\cellcolor{green} $0.22$ &
\cellcolor{green} $0.77$ & 
\cellcolor{green} $2.68$ &
\cellcolor{green} $0.39$ \\
 % \hline
\cellcolor{lightgray}
 Avg. gain over Vanilla KD &
\cellcolor{green} $0.96$ & 
\cellcolor{green} $1.08$ & 
\cellcolor{green} $0.24$ & 
\cellcolor{green} $7.04$ & 
\cellcolor{green} $3.05$ &
\cellcolor{green} $0.93$ \\
  \hline
  
\end{tabular}
}
\end{center}

\vskip -0.2in
\end{table*}


==> tables/crd_dkd.tex <==
\definecolor{beige}{RGB}{245,245,220}


\begin{table*}[h] 
\renewcommand{\arraystretch}{1.15}
\caption{Comparison with CRD and DKD on NLP tasks.}
\label{tab:crd_dkd}

\begin{center}
\tiny

\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{|c| c c c c c c c c|} 
 \hline
 %\rowcolor{cyan}
\cellcolor{cyan}
Teacher & 
ALBERT-Large & 
ALBERT-Large  &
ALBERT-Large & 
ALBERT-XXL &
ALBERT-XXL & 
ALBERT-XXL & 
ALBERT-XXL &
ALBERT-XL
\\ 

 %\hline
 % \rowcolor{cyan}
 \cellcolor{cyan}
Student  & 
ALBERT-Base & 
ALBERT-Base  & 
ALBERT-Base  & 
ALBERT-Base  &
MLP/T5(11B) &
ALBERT-Base  &
MLP/T5(11B) & 
ALBERT-Base \\ 
%\hline
 \cellcolor{cyan}
Dataset&

LMRD&  
GLUE/cola& 
GLUE/sst2 &
Am. Reviews Bin &
Am. Reviews Bin &
Am. Reviews  &
Am. Reviews &
Sentiment140 Bin \\
\hline
 \cellcolor[HTML]{FBB982}
 Teacher & 
 $ 90.19$ &  
 $81.87$ & 
 $ 94.09$ &
 $87.82$ &
 $87.82$ &
 $77.58$ &
 $77.58$ &
 $87.29$ \\

 \hline
\cellcolor[HTML]{FDBC42}
 Vanilla & 
 $ 88.70 \pm 0.17$ &  
 $ 80.50 \pm 0.05 $ & 
 $ 92.39 \pm 0.24$ &
 $86.76 \pm 0.23$ &
 $ 88.6 \pm 0.1 $ &
 $75.13 \pm 0.12 $ &
 $72.30  \pm 1.19 $ &
 $86.14 \pm 0.05 $\\
 
 
 %\hline
 \cellcolor[HTML]{FDBC42}
CRD &   
 $ 89.19 \pm 0.03$ & 
 $ 80.79 \pm 0.21$ & 
 $  92.27 \pm 0.48 $&
 $85.79 \pm 0.11 $ &
 $88.12 \pm 0.91$ &
 $74.7 \pm 1.32$  &
 $61.08 \pm 1.8$  & 
 $84.60 \pm 0.69$ \\
 
 %\hline
 \cellcolor[HTML]{FDBC42}
DKD &   
 — & 
 —  & 
— &
 — &
 — &
 $73.41 \pm  0.35 $&
 $72.41 \pm 0.91$ &
 — \\


 %\hline
 \cellcolor[HTML]{FDBC42}
LELP (Ours) &  
 $\mathbf{89.22 \pm 0.06}$ & 
 $\mathbf{81.43 \pm 0.47}$ & 
 $\mathbf{92.81 \pm 0.36}$ &
$\mathbf{88.49 \pm 0.36}$ &
$\mathbf{91.76 \pm 0.17}$ &
$\mathbf{78.08 \pm 0.81}$ &
$\mathbf{77.48 \pm 0.43}$ &
$\mathbf{87.00 \pm 0.25}$\\
 

\hline
  
\end{tabular}
}
\end{center}


\end{table*}

==> tables/embedding_dimensions.tex <==

\begin{table*}[h] 
\renewcommand{\arraystretch}{1.15}
\label{tab:embeddings_dimension}

\begin{center}
\tiny
\begin{tabular}{|c| c|} 
 \hline
 % \rowcolor{cyan}
% \cellcolor{cyan}
Architecture &  Embeddings Dimension \\ 
\hline
ResNet92  & 256 \\
ResNet56 &  256 \\
MobileNet (Student) & 1024 \\
MobileNet (Teacher) & 2048 \\
ALBERT-Large & 1024  \\
ALBERT-Base & 768 \\ 
\hline
  
\end{tabular}
\end{center}


\end{table*}

==> tables/hyperparameters_fitnet_vid.tex <==
\begin{table*}[h!] 
\renewcommand{\arraystretch}{1.15}

\label{tab:hyperparameters_fitnet_vid}


\centering
\begin{minipage}{0.45\textwidth}

\centering
\caption{Hyperparameters for FitNet}
\tiny
\begin{tabular}{|c| c c|} 
 \hline
 %\rowcolor{cyan}
Dataset
& Temperature
& Embeddings-loss coefficient
\\ 

 \hline
CIFAR-10-bin
& $\{\textbf{1.0}, 2.0, 3.0, 4.0, \emph{5.0}, 10.0\}$  
& $\{0.1, 1.0, 5.0, 10.0, \textbf{100.0}, \emph{1000.0} \}$ \\ 

 \hline
 % \rowcolor{cyan}

CIFAR-100-bin
&  $\{\textbf{1.0}, 2.0, 3.0, 4.0, 5.0, \emph{10.0}\}$  
 & $\{ 0.1, \emph{1.0}, 5.0, 10.0, \textbf{100.0}, 1000.0 \}$ \\ 
\hline


CIFAR-10 
&  $\{\textbf{1.0}, 2.0, 3.0, \emph{4.0}, 5.0, 10.0\}$  
 & $\{0.1, 1.0, \emph{5.0}, 10.0, \textbf{100.0}, 1000.0 \}$ \\ 
\hline


CIFAR-100
&  $\{\textbf{1.0}, 2.0, 3.0, 4.0, \emph{5.0}, 10.0\}$  
 & $\{\emph{0.1}, \textbf{1.0}, 5.0, 10.0, 100.0, 1000.0 \}$ \\ 
\hline


LMRD
&  $\{ \textbf{1.0}, 2.0, 3.0, 4.0, 5.0, 10.0\}$  
 & $\{0.1, \textbf{1.0}, 5.0, 10.0, 100.0, 1000.0 \}$ \\ 
\hline


GLEU/cola 
&  $\{1.0, 2.0, 3.0, 4.0, \textbf{5.0}, 10.0\}$  
 & $\{0.1, 1.0, 5.0, \textbf{10.0}, 100.0, 1000.0 \}$ \\ 
\hline

GLEU/sst 
&  $\{1.0, 2.0, \textbf{3.0}, 4.0, 5.0, 10.0\}$  
 & $\{0.1, 1.0, \textbf{5.0}, 10.0, 100.0, 1000.0 \}$ \\ 
\hline

\end{tabular}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}

\centering
\caption{Hyperparameters for VID}
\tiny
\begin{tabular}{|c| c c|} 
 \hline
 %\rowcolor{cyan}
Dataset
& Temperature
& Embeddings-loss coefficient
\\ 

 \hline
CIFAR-10-bin
& $\{\textbf{1.0}, 2.0, 3.0, 4.0, 5.0, \emph{10.0}\}$  
& $\{ \emph{0.1}, \textbf{0.2},  0.5, 1.0, 5.0, 10.0,  100.0 \}$ \\ 

 \hline
 % \rowcolor{cyan}

CIFAR-100-bin
& $\{1.0, \textbf{2.0}, 3.0, 4.0, \emph{5.0}, 10.0\}$  
& $\{ \textbf{0.1}, 0.2,  \emph{0.5}, 1.0, 5.0, 10.0,  100.0 \}$ \\ 

\hline


CIFAR-10 
& $\{1.0, 2.0, 3.0, \textbf{4.0}, 5.0, \emph{10.0}\}$  
& $\{ \textbf{\emph{0.1}}, 0.2,  0.5, 1.0, 5.0, 10.0,  100.0 \}$ \\ 
\hline


CIFAR-100
& $\{1.0, 2.0, \emph{3.0}, 4.0, 5.0, \textbf{10.0}\}$  
& $\{ \textbf{0.1}, 0.2,  0.5, \emph{1.0}, 5.0, 10.0,  100.0 \}$ \\ 
\hline


LMRD
& $\{ 1.0, 2.0, 3.0, 4.0, 5.0, \textbf{10.0}\}$  
& $\{ \textbf{0.1}, 0.2,  0.5, 1.0, 5.0, 10.0,  100.0 \}$ \\ 
\hline


GLEU/cola 
& $\{1.0, \textbf{3.0}, 3.0, 4.0, 5.0, 10.0\}$  
& $\{ \textbf{0.1}, 0.2,  0.5, 1.0, 5.0, 10.0,  100.0 \}$ \\ 
\hline

GLEU/sst 
& $\{1.0, 2.0, 3.0, 4.0, 5.0, \textbf{10.0}\}$  
& $\{ \textbf{0.1}, 0.2,  0.5, 1.0, 5.0, 10.0,  100.0 \}$ \\ 
\hline

\end{tabular}
\end{minipage}



\end{table*}



==> tables/hyperparams_agglo.tex <==
\begin{table*}[t] 
\renewcommand{\arraystretch}{1.15}

\label{tab:hyperparams_algo}


\centering
\caption{Hyperparameters for Agglomerative Clustering}
\tiny
\begin{tabular}{|c| c |} 
 \hline
 %\rowcolor{cyan}
Dataset
& Number of Clusters \\ 

 \hline
CIFAR-10-bin
& $\{ \textbf{4}, 6, 8, \emph{10}, 20, 50, 100, 1000\}$ \\ 

% \hline
 % \rowcolor{cyan}

CIFAR-100-bin
& $\{ \textbf{10}, 20, 30, 40, 50, 60, \emph{70}, 80, 90, 100, 150, 200\}$ \\ 
\hline


\end{tabular}
\end{table*}


==> tables/hyperparams_kmeans.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.15}
\centering
\caption{Hyperparameters for K-Means Clustering}
\tiny
\begin{tabular}{|c| c |} 
 \hline
 %\rowcolor{cyan}
Dataset
& Number of Clusters \\ 

 \hline
CIFAR-10-bin
& $\{ 4, \emph{6}, 8, \textbf{10}, 20, 50, 100, 1000\}$ \\ 

% \hline
 % \rowcolor{cyan}

CIFAR-100-bin
& $\{ \textbf{10}, 20, 30, 40, \emph{50}, 60, 70, 80, 90, 100, 150, 200\}$ \\ 
\hline


\end{tabular}

\end{table*}

==> tables/hyperparams_tsne_kmeans.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.15}

\label{tab:hyperparameters_tsne_kmeans}


\centering
\caption{Hyperparameters for  t-SNE \& K-Means Clustering}
\tiny
\begin{tabular}{|c| c |} 
 \hline
 %\rowcolor{cyan}
Dataset
& Number of Clusters \\ 

 \hline
CIFAR-10-bin
& $\{ 2, \textbf{3}, \emph{4}, 5, 10, 25, 50, 500\}$ \\ 

% \hline
 % \rowcolor{cyan}

CIFAR-100-bin
& $\{ \textbf{\emph{5}}, 10, 15, 20, 25, 30, 35, 40, 45, 50, 75, 100\}$ \\ 
\hline


\end{tabular}
\end{table*}

==> tables/t5mlp.tex <==


\definecolor{beige}{RGB}{245,245,220}


\begin{table*}[h] 
\renewcommand{\arraystretch}{1.15}
\caption{NLP experiments using MLPs over T5-representations}
\label{tab:nlp_t5}

\begin{center}
\tiny
\begin{tabular}{|c| c c|} 
 \hline
 %\rowcolor{cyan}
\cellcolor{cyan}
Teacher Architecture & 
ALBERT-XXL & 
ALBERT-XXL 
\\ 

 %\hline
 % \rowcolor{cyan}
 \cellcolor{cyan}
Student Architecture  & 
MLP/T5(11B) &
MLP/T5(11B) \\ 
%\hline
 \cellcolor{cyan}
Dataset&

Am. Reviews Bin &
Am. Reviews \\
\hline
 \cellcolor[HTML]{FBB982}
 Teacher & 
 $87.82$ &
 $77.58$ \\
%\hline
 \cellcolor[HTML]{FBB982}
 Subclass Distillation Teacher& 
 $87.53$ &
 $78.02$ \\


\hline
\cellcolor[HTML]{FDBC42}
Standard Training & 
 $87.83 \pm 1.48$ & 
$ 66.44 \pm 0.23$  \\

 
 
 %\hline
\cellcolor[HTML]{FDBC42}
 Vanilla Distillation & 
 $ 88.6 \pm 0.1 $ &
 $72.30  \pm 1.19 $ \\
 
 
 %\hline
 \cellcolor[HTML]{FDBC42}
 Embedding Distillation &   
 $89.84 \pm 0.78$ &
 $72.64 \pm 0.95$ \\
 
 %\hline
 \cellcolor[HTML]{FDBC42}
 FitNet &   
 $\underline{91.4 \pm 0.5}$ &
 $75.78 \pm 0.21$ \\

 %\hline
 \cellcolor[HTML]{FDBC42}
 VID  & 
$89.23 \pm 0.91 $ &
$63.98 \pm 1.79 $  \\
 %\hline
 \cellcolor[HTML]{FDBC42}
 Relational KD  & 
 $89.52 \pm 0.95 $ &
$74.72 \pm 0.79$ \\


 \cellcolor[HTML]{FDBC42}
 DKD  & 
 $88.6 \pm 0.1 $ &
$72.41 \pm 0.91$ \\


 \cellcolor[HTML]{FDBC42}
 CRD  & 
 $88.12 \pm 0.91 $ &
$61.08 \pm 1.8$ \\


 \cellcolor[HTML]{FDBC42}
 Subclass Distillation  &  
 $90.38 \pm 0.82$ &
 $\underline{77.27 \pm 1.45}$  \\

 %\hline
 \cellcolor[HTML]{FDBC42}
LELP (Ours) &  
$\mathbf{91.76 \pm 0.17}$ &
$\mathbf{77.48 \pm 0.43}$ \\
 
 \hline
  \cellcolor{lightgray}
 Avg. gain over the best baseline &
\cellcolor{green} $0.36$ & 
\cellcolor{green} $0.21$ \\ 

% \hline
  \cellcolor{lightgray}
 Avg. gain over non-subclass baseline &
\cellcolor{green} $0.36$ & 
\cellcolor{green} $1.68$ \\ 

 % \hline
\cellcolor{lightgray}
 Avg. gain over Vanilla KD&
\cellcolor{green} $3.16$ &
\cellcolor{green} $5.18$ \\

\hline
  
\end{tabular}
\end{center}


\end{table*}

==> tables/vision_and_nlp.tex <==
\definecolor{beige}{RGB}{245,245,220}
\begin{table*}[h] 
\renewcommand{\arraystretch}{1.15}
\caption{Experiments on \textbf{Vision Multi-Classification} and \textbf{Binary NL Classification} tasks.}
\label{tab:multiclass}

\begin{center}
\tiny
\begin{tabular}{|c| c c c c c c c |} 
 \hline
 %\rowcolor{cyan}
\cellcolor{cyan}
Teacher Architecture 
& ResNet92 
& ResNet92
& ResNet92
& ResNet92 
&ALBERT-Large 
&ALBERT-Large  
&ALBERT-Large
\\ 

% \hline
 % \rowcolor{cyan}
 \cellcolor{cyan}
Student Architecture& 
ResNet56 &  
MobileNet  & 
ResNet56  & 
MobileNet &
ALBERT-Base & 
ALBERT-Base  & 
ALBERT-Base 
\\ 
%\hline
 \cellcolor{cyan}
Dataset&
CIFAR-10&  
CIFAR-10& 
CIFAR-100& 
CIFAR-100 &
LMRD&  
GLUE/cola& 
GLUE/sst2 \\ 
\hline
 \cellcolor[HTML]{FBB982}
 Teacher & 
 $ 94.94$ &  
 $94.94$ & 
 $ 75.55 $ & 
 $ 75.55$ &
 $ 90.19$ &  
 $81.87$ & 
 $ 94.09$ \\
%\hline
 \cellcolor[HTML]{FBB982}
 Subclass Distillation Teacher
 & 
 $ 93.79 $ &  
 $93.49 $ & 
 $ 73.79 $ & 
 $ 70.23 $ &
  $ 90.05 $ &  
 $81.49 $ & 
 $ 93.11 $ 
 \\
\hline
\cellcolor[HTML]{FDBC42}
Standard Training & 
 $ 93.02 \pm 0.11$ &  
 $ 84.86 \pm 0.11 $ & 
 $ 72.53 \pm 0.18 $ & 
 $ 53.15 \pm 0.21$ &
  $ 87.68 \pm 0.46$ &  
 $ 79.13 \pm 0.79 $ & 
 $ 91.32 \pm 0.12$ \\
 
% \hline
\cellcolor[HTML]{FDBC42}
 Vanilla Distillation & 
 $ 93.49 \pm 0.32$ &  
 $ 86.45 \pm 0.21 $ & 
 $ 76.31 \pm 0.14 $ & 
 $ 56.20 \pm 0.11$ &
  $ 88.70 \pm 0.17$ &  
 $ 80.50 \pm 0.05 $ & 
 $ 92.39 \pm 0.24$ \\
 
 
% \hline
 \cellcolor[HTML]{FDBC42}
 Embedding Distillation &   
 $94.43 \pm 0.08$  & 
 $86.82 \pm 0.16$ & 
 $76.47 \pm 0.1$ & 
 $57.27 \pm 0.4$ &
  $ 88.98 \pm 0.33$ & 
 $ 80.66 \pm 0.65$ & 
 $  92.62 \pm 0.16 $\\
 
% \hline
 \cellcolor[HTML]{FDBC42}
 FitNet &   
 $ \mathbf{94.61 \pm 0.04}$ & 
 $ 85.70 \pm 0.36$ & 
 $ 76.49 \pm 0.37$ & 
 $  38.23 \pm 1.12 $&
  $ 88.75 \pm 0.15$ & 
 $ 80.82 \pm 0.32$ & 
 $  92.43 \pm 0.18$\\
% \hline
 \cellcolor[HTML]{FDBC42}
 VID  & 
 $94.51 \pm 0.12$ & 
 $76.36 \pm 1.56$ & 
 $76.20 \pm 0.29$ & 
 $27.08 \pm 1.08$ &
  $88.26 \pm 0.20$ & 
 $79.83 \pm 0.62$ & 
 $91.47 \pm 0.33$ \\  
% \hline
 \cellcolor[HTML]{FDBC42}
 Subclass Distillation &  
 $93.66 \pm 0.04$ & 
 $86.55 \pm 0.28$ & 
 $74.47 \pm 0.07$ & 
 $54.45 \pm 1.25$ &
  $\mathbf{89.24 \pm 0.31}$ & 
 $80.85 \pm 0.1$ & 
 $\mathbf{92.85 \pm 0.15}$ \\
% \hline
 \cellcolor[HTML]{FDBC42}
LELP (Ours) &  
 $94.29 \pm 0.12$ & 
 $\mathbf{88.02 \pm 0.19}$ & 
 $\mathbf{76.66 \pm 0.28}$ & 
 $\mathbf{61.98 \pm 0.08}$ &
  $\mathbf{89.22 \pm 0.06}$ & 
 $\mathbf{81.43 \pm 0.47}$ & 
 $\mathbf{92.81 \pm 0.36}$ \\
 \hline
  \cellcolor{lightgray}
 Avg. gain over the best baseline &
\cellcolor{red} $-0.32$ & 
\cellcolor{green} $1.4$ & 
\cellcolor{green} $0.17$ & 
\cellcolor{green} $4.71$ &
\cellcolor{beige} $-0.02$ & 
\cellcolor{green} $0.58$ & 
\cellcolor{beige} $-0.04$ \\
 % \hline
\cellcolor{lightgray}
 Avg. gain over Vanilla KD &
\cellcolor{green} $0.8$ & 
\cellcolor{green} $1.57$ & 
\cellcolor{green} $0.35$ & 
\cellcolor{green} $5.78$ &
\cellcolor{green} $0.52$ & 
\cellcolor{green} $0.93$ & 
\cellcolor{green} $0.42$ \\
  \hline
  
\end{tabular}
\end{center}


\end{table*}
